Handwritten Code Recognition for Pen-and-Paper CS Education

Teaching Computer Science (CS) by having students write programs by hand on paper has key pedagogical advantages: It allows focused learning and requires careful thinking compared to the use of Integrated Development Environments (IDEs) with intelligent support tools or "just trying things out". The familiar environment of pens and paper also lessens the cognitive load of students with no prior experience with computers, for whom the mere basic usage of computers can be intimidating. Finally, this teaching approach opens learning opportunities to students with limited access to computers. However, a key obstacle is the current lack of teaching methods and support software for working with and running handwritten programs. Optical character recognition (OCR) of handwritten code is challenging: Minor OCR errors, perhaps due to varied handwriting styles, easily make code not run, and recognizing indentation is crucial for languages like Python but is difficult to do due to inconsistent horizontal spacing in handwriting. Our approach integrates two innovative methods. The first combines OCR with an indentation recognition module and a language model designed for post-OCR error correction without introducing hallucinations. This method, to our knowledge, surpasses all existing systems in handwritten code recognition. It reduces error from 30\% in the state of the art to 5\% with minimal hallucination of logical fixes to student programs. The second method leverages a multimodal language model to recognize handwritten programs in an end-to-end fashion. We hope this contribution can stimulate further pedagogical research and contribute to the goal of making CS education universally accessible. We release a dataset of handwritten programs and code to support future research at https://github.com/mdoumbouya/codeocr

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> prev_draft.tex <==
% \subsection{Introduction}
% \input{prev_draft/intro}

% \subsection{Code Digitalization Challenge}
% \input{prev_draft/evaluation}

% \subsection{Methods}
% \input{prev_draft/methods}

\subsection{Results}
\input{prev_draft/results}


% \input{prev_draft/discussion}




==> prev_draft/conclusion.tex <==
todo

==> prev_draft/discussion.tex <==
\subsection{Discussion}
Our research into the digitization of handwritten code, utilizing a symbiotic approach that combines Optical Character Recognition (OCR) with Large Language Models (LLMs), has culminated in both noteworthy outcomes and a comprehensive understanding of the prevailing challenges in this domain. This initiative primarily aimed to augment computer science education in regions where computer accessibility is restricted. The real-world classroom implementation of our system further illuminated its tangible implications and potential.



\subsection{Use in a Low-Resource Classroom}

% Envision a classroom scenario characterized by limited technological resources: twenty students led by a single instructor, with only a solitary smartphone at their disposal. In such an environment, handwritten code offers an innovative solution. Students can meticulously craft their code on paper and, once confident in their solution, leverage the available smartphone for testing. This approach resonates with the time-sharing methodologies employed by earlier mainframe computers, where multiple users could efficiently utilize a singular computing resource in a sequential manner. Such a paradigm not only maximizes resource utility but also encourages students to refine and review their code before digital execution.

% Broadening our perspective, the magnitude of this scenario is significant. According to data from various educational agencies, there are millions of students across developing regions and underprivileged communities globally who face a stark scarcity of digital resources. The scenario illustrated isn't just a theoretical construct, but a real-life situation in many parts of the world. By introducing and scaling such an approach, we can potentially democratize computer science education, ensuring that access to knowledge isn't restricted by access to digital devices.

% Furthermore, such a methodological shift could have cascading benefits on the broader educational landscape. Cultivating a habit of reflection, review, and precision in students can instill qualities that transcend coding, promoting a more deliberate and thoughtful learning approach. Additionally, by embracing such accessible methodologies, educators worldwide can develop curricula that prioritize understanding and problem-solving over mere access to technology. In the long run, this could dramatically level the playing field, providing a strong foundation for underrepresented and underserved students to pursue advanced studies and careers in technology, thereby bridging the global digital divide.



\subsection{Application in Grading Handwritten Exams}

In the current academic landscape, digital exams are susceptible to misconduct, especially with the advent of sophisticated LLMs like ChatGPT. Many educational institutions, from high schools to universities, resort to handwritten exams. These exams, while reducing cheating opportunities, are labor-intensive to grade. Additionally, the potential introduction of gender bias during grading—stemming from handwriting perception—is a concern. By digitizing and accurately recognizing text from these handwritten exams, automated unit tests can be employed. This not only expedites the grading process but also diminishes human-induced grading variance. However, to maintain academic integrity, it's paramount that the digitization process avoids any form of solution hallucination.

\subsection{Benefits of coding without a computer}

- finally, we hope that this tool can be useful in all classrooms.
- somewhat suprising, but many computer science courses already ask students to handwrite code for the simple fact that it can help clarify thinking
- many benefits of handwriting for example:
- one suprising benefit is that students can code without all the other distractions that often accompany using a computer or especially a smart phone. Especially the internet, social media and games. 
- too much screen time can be unhealthy for kids. [todo expand]
- AI can help take us a step towards education that does not need to be mediated by a screen.

\subsection{Grid Base coding}

Grid based coding has been proposed for accesible cs education
https://acrobat.adobe.com/id/urn:aaid:sc:VA6C2:6c1a622c-2ae5-4201-aede-7b37d4a0fc61

Could this be used with graphing paper? Would that be 100\% accurate?

\subsection{Future Directions}

\subsubsection{Working without internet}

todo

Our system's current iteration showcases significant potential, but there's an evident path for further refinement. Delving into advanced LLM architectures, expanding the dataset to cover a wider array of handwriting styles, and implementing automated quality assessments for input images are just a few potential directions. 

In sum, this research emphasizes the transformative potential of harnessing cutting-edge technologies to make computer science education more universally attainable.


==> prev_draft/intro.tex <==
%What is the problem?
A system that enables digitizing handwritten code with high fidelity could enable great educational value. Unfortunately, no such system exists to date.

%$Why is it interesting and important?
The ability to automatically digitize handwritten code can power novel, and perhaps more pedagogical CS education scenarios, as well as make CS education more accessible in certain settings.

% Why is it hard? (E.g., why do naive approaches fail?)
Reasons for the difficulty of automatic digitization mainly lie in the variability in handwriting styles, legibility, and imaging conditions. Second, for programming languages where indentation levels are part of the language syntax such as Python, correctly recognizing handwritten indentation levels add to the difficulty.

%Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
Language models have previously been used to post-correct the output of various recognition systems, including optical character recognition and speech recognition. In the case of handwritten code recognition, a language model that captures the distribution of code is necessary. We hypothesize that the post-correction of handwritten code can be done with large language models. The generative power of large language models can hinder the fidelity of the overall system's output to the input handwritten text. We show that this fidelity can be controlled by means of appropriately prompting large language models.


% What are the key components of my approach and results? Also include any specific limitations.
(1) release of a new dataset for evaluating handwriten code difitization systems.
(2) A method of post-correcting OCR systems with large language models with controllable fidelity.
(3) A formative study in which the use of this technology in real classrooms is evaluated.



\subsection{Notes}
\begin{enumerate}
    \item Handwriting to Digitized Code is an important and hard problem
    \item We discovered that adding an LLM to microsoft azure we can substantially decrease error rates. We show that this introduces minimal 
    \item We experiment with a few different settings and see rather stable results
    \item We discuss opportunities to automatically detect python indentation
\item We discuss ways to achieve 100\% accuracy using a graph paper

\end{enumerate}

\subsection{Major Contributions}
\begin{enumerate}
    \item \textbf{Posed an evaluation for handwriting to digitized code}
    Provide an open source dataset.
    \item \textbf{Provide a novel method of OCR for handwritten code} Combine Microsoft Azure with LLMs. Achieves 5\% error rate, an improvement from the 30.8\% error 
    \item \textbf{Test in a real world classroom} Bangladesh classroom with 7 students.
\end{enumerate}



\subsection{Related Work}
\input{prev_draft/related}


==> prev_draft/methods.tex <==
\subsection{Code Edit Distance}

In the realm of evaluating Optical Character Recognition (OCR) algorithms, understanding how closely the digitalization from the algorithm approximates the true gold label digitalization is crucial. One effective metric to measure this disparity is the edit distance, often known as the Levenshtein distance. This metric quantifies the minimal number of single-character edits (i.e., insertions, deletions, or substitutions) required to change one word into another.

By computing the edit distance, we obtain a tangible measure of the OCR algorithm's accuracy relative to the true gold label digitalization. Lower values of the edit distance indicate that the algorithm's output is closer to the gold standard, and conversely, higher values suggest more discrepancies.

We open source a collection of 40 programs handwritten by students in a CS1 course and a gold label digitalization for each program. The tasks range from X to Y.

\subsection{Solution Hallucination Test}

One of the primary concerns in integrating AI systems that possess vast knowledge of coding is the potential risk of the system inadvertently providing answers to the students. Take, for example, a scenario wherein a student is attempting to write a solution to the Fibonacci sequence, a rather standard programming task. An AI system, especially one equipped with a language model layer, might unintentionally rectify conceptual errors in the student's code, leading to what we term as ``solution hallucination''. This not only risks undermining the student's learning process but also doesn't represent a good faith translation of the student's original intention.

To safeguard against this and to accurately measure the extent of solution hallucination, a robust testing method is essential. In response to this need, we introduced the \textit{Deliberate Error Dataset}. This dataset comprises a curated selection of typical student errors, thereby serving as a benchmark to determine whether the AI recognition algorithm tends to hallucinate fixes.

The Deliberate Error Dataset includes 10 programs. Each program has an image of the program handwritten, the correct digitalization, and the solution to the error (which should not be given away). The dataset contains a spectrum of errors such as:

\begin{itemize}
    \item Fence Post Error
    \item Arithmetic Error
    \item Control Flow Error
    \item Scope Error
\end{itemize}

To ensure the integrity and validity of our tests, hand labelling of the errors from this dataset is performed blindly, without prior knowledge of which algorithm was responsible for producing the digitalization. Such a blind approach negates potential biases and eliminates threats to the study's validity.


==> prev_draft/related.tex <==


Over the years, several attempts have been made to address the challenges of making computer science education more accessible, especially in areas with limited access to computer systems. Additionally, recognizing and digitizing handwritten texts, particularly code, has been a subject of study with its unique challenges.

\paragraph{Computer Science Education without Computers}

Several initiatives  have explored the teaching of computer science principles without the need for physical computers. Approaches such as the CS Unplugged  use off-computer activities to teach core concepts. However, the lack of an execution environment remains a challenge.

\paragraph{Handwriting Recognition and Digitization}

Handwritten document digitization primarily revolves
around Optical Character Recognition (OCR) systems  Various OCR systems have been developed over the years, with some designed specifically for challenging tasks like ancient manuscript digitization 

The task of recognizing handwritten code, however, poses additional challenges. The importance of syntax-specific indentations and unique coding symbols requires more than a typical OCR solution 

\paragraph{Large Language Models in OCR}

Integrating Large Language Models (LLMs) with OCR for post-correction has gained traction recently. Previous works  hint at the potential of LLMs in this domain but rarely target the specific challenges presented by handwritten code.

\paragraph{Datasets for Handwritten Recognition}

While numerous datasets for handwritten document recognition exist very few cater to handwritten code. The scarcity of such datasets limits the advancement of technologies tailored for this niche domain.

In conclusion, while each of these related domains offers valuable insights, our work bridges the gaps between them, introducing a comprehensive solution for digitizing handwritten code, making computer science education more universally accessible.



==> prev_draft/results.tex <==
\input{prev_draft/exp_results}


% \begin{table*}
%     \centering
%     \begin{tabular}{ccccccccc}
%     \toprule
%         Model & Google OCR & AWS & MathPix & Azure & Simple Prompt & COT Prompt & Indentation Recognition + COT\\
%     \midrule
%         Edit Distance & $39.44 \pm 3.57$\% & $34.43 \pm 2.31$\% & $64.6 \pm 5.5$\% & $30.53 \pm 1.62$\% & $6.1 \pm 1.32$\% & $6.66 \pm 1.91$\% & $15.18 \pm 0.16$\% \\
%         Mean & 39.44\% & 34.43\% & 64.6\% & 30.53\% & 6.1\% & 6.66\% & 15.18\% \\
%         Std Deviation & 26.2\% & 16.99\% & 40.45\% & 11.88\% & 9.67\% & 14.06\% & 9.99\%\\
%         Std Error & 3.57\% & 2.31\% & 5.5\% & 1.62\% & 1.32\% & 1.91\% & 0.16\% \\
%     \bottomrule
%     \end{tabular}
%     \caption{Benchmark of all the OCR (with comments in code) (n = 55)}
% \end{table*}

% \begin{figure*}
% \centering
% \includegraphics[width=\textwidth]{prev_draft/figures/withcommentbar.png}
% \caption{Bar Chart of benchmark of OCR (Code with comment)}
% \label{1}
% \end{figure*}


\begin{table*}
    \centering
    \begin{tabular}{l|cccc} 
    \hline
        Errors/Prompting & Double Prompting & Low & Medium & High \\ 
    \hline
        No Change &                               60\% & 56.36\% & 50.91\% & 52.73\% \\
        Small Change in the Comment &           7.27\% &  3.64\% &  5.45\% &  3.64\% \\
        Missed Something From Ground Truth &    3.64\% &     0\% &     0\% &     0\% \\
        Print Statement Change &                1.82\% &  1.82\% &  1.82\% &  1.82\% \\
        Added code that was not present &          0\% &  1.82\% &  3.64\% &  1.82\% \\
        Small Variable/Function Name Change &  14.55\% &  9.09\% & 12.73\% & 10.91\% \\
        Small Change in the Indentation &       7.27\% &  5.45\% &  5.45\% &  5.45\% \\
        Small Syntax Fix &                      5.45\% &  9.09\% &  9.09\% &  9.09\% \\
        Logical Fix &                              0\% & 12.73\% & 10.91\% & 14.55\% \\
    \hline
    \end{tabular}
    \caption{Comparison of Hallucination in different prompting techniques (n=55)}
\end{table*}


\begin{table*}
    \centering
    \begin{tabular}{l|cc} 
    \hline
        Errors & Definitions \\ 
    \hline
        No/Minimal Change &                     Output Same as Ground Truth, or very minimal modification in whitespace \\
        Small Change in the Comment &           Minor Modifications or Syntax Alterations in Code Comments \\
        Missed Something From Ground Truth &    Neglected information present in Image\\
        Print Statement Change &                Modified the string inside the print statement\\
        Added code that was not present &       Added Extra Code Not Present in the Image, without Impacting Code Logic\\
        Small Variable/Function Name Change &  Modified the name of the variable/function, without impacting code logic\\
        Small Change in the Indentation &       Modified indentation for out-of-distribution code, Negatively Affecting Functionality\\
        Small Syntax Fix &                      Corrected minor syntax errors, including in-built function case and statement interchange\\
        Logical Fix &                           Corrected logical errors that improves Code functionality, and lead to answer, or gives away the answer\\
    \hline
    \end{tabular}
    \caption{Comparison of Hallucination in different prompting techniques (n=55)}
\end{table*}



